Finite-Time Error Bounds for Distributed Linear Stochastic Approximation

This paper considers a novel multi-agent linear stochastic approximation algorithm driven by Markovian noise and general consensus-type interaction, in which each agent evolves according to its local stochastic approximation process which depends on the information from its neighbors. The interconnection structure among the agents is described by a time-varying directed graph. While the convergence of consensus-based stochastic approximation algorithms when the interconnection among the agents is described by doubly stochastic matrices (at least in expectation) has been studied, less is known about the case when the interconnection matrix is simply stochastic. For any uniformly strongly connected graph sequences whose associated interaction matrices are stochastic, the paper derives finite-time bounds on the mean-square error, defined as the deviation of the output of the algorithm from the unique equilibrium point of the associated ordinary differential equation. For the case of interconnection matrices being stochastic, the equilibrium point can be any unspecified convex combination of the local equilibria of all the agents in the absence of communication. Both the cases with constant and time-varying step-sizes are considered. In the case when the convex combination is required to be a straight average and interaction between any pair of neighboring agents may be uni-directional, so that doubly stochastic matrices cannot be implemented in a distributed manner, the paper proposes a push-sum-type distributed stochastic approximation algorithm and provides its finite-time bound for the time-varying step-size case by leveraging the analysis for the consensus-type algorithm with stochastic matrices and developing novel properties of the push-sum algorithm. Distributed temporal difference learning is discussed as an illustrative application.

==> Analysis_and_Proofs.tex <==
\section{Analysis and Some Proofs}\label{analysis}

In this appendix, we provide the analysis of our two algorithms, \eqref{eq:theta update} and \eqref{eq:SA_push-sum}, and the proofs of all the assertions in the paper. We begin with some notation used in the analysis.


\subsection{Notation}
\input{Appendix_notation}

\subsection{Distributed Stochastic Approximation}\label{proofs:sa}

In this subsection, we analyze the distributed stochastic approximation algorithm \eqref{eq:theta update} and provide the proofs of the results in Section~\ref{sec:SA}. 
We begin with the asymptotic performance. 

{\color{black}
{\bf Proof of Theorem~\ref{thm:consensus_time-varying_jointly}:}
Without loss of generality, let $\{\bbb{G}_t\}$ be uniformly strongly connected by sub-sequences of length $L$.
Note that for any $i\in\mathcal{V} $, 
\begin{align}\label{eq:proof_th1_1_jointly}
    0 &\le \pi_{\min}\|\theta^i_t-\langle \theta\rangle_t\|_2^2 \le \pi_{\min} \sum_{j=1}^N \|\theta^j_t-\langle \theta\rangle_t\|_2^2 \nonumber\\
    &\le \sum_{j=1}^N \pi_t^j \|\theta^j_t-\langle \theta\rangle_t\|_2^2,
\end{align}
where $\pi_{\min}$ is defined in Lemma~\ref{lemma:bound_pi_jointly}. From Lemma~\ref{lemma:bound_consensus_time-varying_jointly}, 
\begin{align} \label{eq:proof_th1_2_jointly}
    &\lim_{t\to\infty}\sum_{i=1}^N \pi_{t}^i \| \theta_{t}^i - \langle \theta \rangle_{t} \|_2^2 \nonumber\\
    \le \; &  \lim_{t\to\infty}\hat \epsilon^{q_t - {T_4^*}} \sum_{i=1}^N \pi_{T_4^*L+m_t}^i \| \theta_{T_4^*L+m_t}^i - \langle \theta \rangle_{T_4^*L+m_t} \|_2^2 \nonumber \\
    &+ \lim_{t\to\infty} \frac{\zeta_6}{1-\hat\epsilon} \left( \alpha_0 \hat\epsilon^{\frac{q_t-1}{2}} + \alpha_{\ceil{\frac{q_t-1}{2}}L} \right) \nonumber\\
    =\;& 0. 
\end{align}
Combining \eqref{eq:proof_th1_1_jointly} and \eqref{eq:proof_th1_2_jointly}, it follows that for all $i\in\mathcal{V}$, $\lim_{t\to\infty} \pi_{\min}\|\theta^i_t-\langle \theta\rangle_t\|_2^2 = 0$. 
Since $\pi_{\min}>0$ by Lemma~\ref{lemma:bound_pi_jointly}, $\lim_{t\to\infty} \|\theta^i_t-\langle \theta\rangle_t\|_2 = 0$ for all $i\in\mathcal{V}$.
\hfill$\qed$}





%\noindent
{\bf Proof of Theorem~\ref{thm:theta^*_jointly}:}
%{\color{red}Part (1) can be proved by specialization of Theorem~3.1 in \cite{kushner87}.}
From Theorem~\ref{thm:consensus_time-varying_jointly}, all $\theta_t^i$, $i\in \mathcal{V}$, will reach a consensus with $ \langle \theta \rangle_t $ and the update of $ \langle \theta \rangle_t $ is given in \eqref{eq:update of average_time-varying}, which can be treated as a single-agent linear stochastic approximation whose corresponding ODE is \eqref{eq:definition theta^*}.
From \cite{kushner87, kushner1983averaging},\footnote{On page 1289 of \cite{kushner87}, it says that the idea in \cite{kushner1983averaging} can be adapted to get the w.p.1 convergence result.
} 
we know that $ \langle \theta \rangle_t $ will converge to $\theta^*$ w.p.1, which implies that $\theta_t^i$ will converge to $\theta^*$ w.p.1. 
In addition, from Theorem~\ref{thm:bound_jointly_SA}-(2) and Lemma~\ref{lemma:eta_sum}, 
$\lim_{\rightarrow\infty}\sum_{i=1}^N \pi_t^i \mathbf{E}[\|\theta_t^i - \theta^*\|_2^2]=0$. Since $\pi_t^i$ is uniformly bounded below by $\pi_{\min}>0$, as shown in Lemma~\ref{lemma:bound_pi_jointly}, 
it follows that $\theta_t^i$ will converge to $\theta^*$ in mean square for all $i\in\mathcal{V}$.
\hfill $\qed$




We now analyze the finite-time performance of \eqref{eq:theta update}. In the sequel, we use $K$ to denote the dimension of each $\theta_t^i$, i.e., $\theta_t^i \in \R^K$ for all $i\in\mathcal{V}$.

\input{Proof_jointly}

\subsection{Push-SA}\label{proofs:push}


In this subsection, we analyze the push-based distributed stochastic approximation algorithm \eqref{eq:SA_push-sum} and provide the proofs of the results in Section~\ref{sec:SA_pushsum}. 


%We begin with the proof of asymptotic performance of \eqref{eq:SA_push-sum}. 



%%\noindent
%{\bf Proof of Theorem~\ref{thm:push_meansq}:}
%%{\color{red}Part (1) can be proved by specialization of Theorem~3.1 in \cite{kushner87}.}
%From Lemma~\ref{lemma:bound_consensus_time-varying_push_SA}, since $\bar \epsilon \in(0,1)$ and $\alpha_t = \frac{\alpha_0}{t}$, we have $\lim_{t\to\infty}\| \theta_{t+1}^i - \langle \tilde \theta \rangle_t \|_2 = 0$, which implies that all $\theta_{t+1}^i$, $i\in \mathcal{V}$, will reach a consensus with $ \langle \tilde \theta \rangle_t $. The update of $ \langle \tilde \theta \rangle_t $ is given in \eqref{eq:update_average_tilde_theta}, which can be treated as a single-agent linear stochastic approximation whose corresponding ODE is \eqref{eq:ode_pushsum}. In addition, from Theorem~\ref{thm:bound_time-varying_step_Push_SA} and Lemma~\ref{lemma:eta_limit_Push_SA}, $\lim_{\rightarrow\infty}\sum_{i=1}^N \mathbf{E}[\|\theta_{t+1}^i - \theta^*\|_2^2]=0$, it follows that $\theta_{t+1}^i$ will converge to $\theta^*$ in mean square for all $i\in\mathcal{V}$.
%\hfill $\qed$

%\vspace{.1in}

{\color{black}
We begin with the analyses of the finite-time performance of algorithm \eqref{eq:SA_push-sum}.
%We next analyze the finite-time performance of \eqref{eq:SA_push-sum}. 
}


\input{Proof_push} \label{sec:proof_push}

==> Analysis_and_Proofs_full.tex <==
\section{Analysis and Proofs}\label{analysis}

In this appendix, we provide the analysis of our two algorithms, \eqref{eq:theta update} and \eqref{eq:SA_push-sum}, and the proofs of all the assertions in the paper. We begin with some notation.


\subsection{Notation}
\input{Appendix_notation}

\subsection{Distributed Stochastic Approximation}\label{proofs:sa}

In this subsection, we analyze the distributed stochastic approximation algorithm \eqref{eq:theta update} and provide the proofs of the results in Section~\ref{sec:SA}.
We begin with the asymptotic performance. 







%\noindent
{\bf Proof of Theorem~\ref{thm:theta^*_jointly}:}
%{\color{red}Part (1) can be proved by specialization of Theorem~3.1 in \cite{kushner87}.}
From Theorem~\ref{thm:consensus_time-varying_jointly}, all $\theta_t^i$, $i\in \mathcal{V}$, will reach a consensus with $ \langle \theta \rangle_t $ and the update of $ \langle \theta \rangle_t $ is given in \eqref{eq:update of average_time-varying}, which can be treated as a single-agent linear stochastic approximation whose corresponding ODE is \eqref{eq:definition theta^*}.
From \cite{kushner87, kushner1983averaging},\footnote{On page 1289 of \cite{kushner87}, it says that the idea in \cite{kushner1983averaging} can be adapted to get the w.p.1 convergence result.
} 
we know that $ \langle \theta \rangle_t $ will converge to $\theta^*$ w.p.1, which implies that $\theta_t^i$ will converge to $\theta^*$ w.p.1. 
In addition, from Theorem~\ref{thm:bound_jointly_SA}-(2) and Lemma~\ref{lemma:eta_sum}, 
$\lim_{\rightarrow\infty}\sum_{i=1}^N \pi_t^i \mathbf{E}[\|\theta_t^i - \theta^*\|_2^2]=0$. Since $\pi_t^i$ is uniformly bounded below by $\pi_{\min}>0$, as shown in Lemma~\ref{lemma:bound_pi_jointly}, 
it follows that $\theta_t^i$ will converge to $\theta^*$ in mean square for all $i\in\scr V$.
\hfill $\qed$




We now analyze the finite-time performance of \eqref{eq:theta update}. In the sequel, we use $K$ to denote the dimension of each $\theta_t^i$, i.e., $\theta_t^i \in \R^K$ for all $i\in\scr V$.

\input{Proof_jointly}

\subsection{Push-SA}\label{proofs:push}


In this subsection, we analyze the push-based distributed stochastic approximation algorithm \eqref{eq:SA_push-sum} and provide the proofs of the results in Section~\ref{sec:SA_pushsum}. We begin with the proof of asymptotic performance of \eqref{eq:SA_push-sum}. 

%\noindent
{\bf Proof of Theorem~\ref{thm:push_meansq}:}
%{\color{red}Part (1) can be proved by specialization of Theorem~3.1 in \cite{kushner87}.}
From Lemma~\ref{lemma:bound_consensus_time-varying_push_SA}, since $\bar \epsilon \in(0,1)$ and $\alpha_t = \frac{\alpha_0}{t}$, we have $\lim_{t\to\infty}\| \theta_{t+1}^i - \langle \tilde \theta \rangle_t \|_2 = 0$, which implies that all $\theta_{t+1}^i$, $i\in \mathcal{V}$, will reach a consensus with $ \langle \tilde \theta \rangle_t $. The update of $ \langle \tilde \theta \rangle_t $ is given in \eqref{eq:update_average_tilde_theta}, which can be treated as a single-agent linear stochastic approximation whose corresponding ODE is \eqref{eq:ode_pushsum}.
In addition, from Theorem~\ref{thm:bound_time-varying_step_Push_SA} and Lemma~\ref{lemma:eta_limit_Push_SA}, 
$\lim_{\rightarrow\infty}\sum_{i=1}^N \mathbf{E}[\|\theta_{t+1}^i - \theta^*\|_2^2]=0$, it follows that $\theta_{t+1}^i$ will converge to $\theta^*$ in mean square for all $i\in\scr V$.
\hfill $\qed$

\vspace{.1in}

We next analyze the finite-time performance of \eqref{eq:SA_push-sum}.


\input{Proof_push} \label{sec:proof_push}

==> Proof_jointly.tex <==
\subsubsection{Fixed Step-size} \label{sec:proof_jointly_fixed}


We first consider the fixed step-size case and begin with validation of two ``convergence rates'' in Theorem~\ref{thm:bound_jointly_SA}. 


\begin{lemma}\label{lemma:ration_in_0_1}
    Both $\epsilon$ and $(1-\frac{0.9 \alpha}{\gamma_{\max}})$ lie in the interval $(0,1)$.
\end{lemma}







%From the definition of $\zeta_1$ in Section~\ref{sec:constants} and Remark~\ref{remark:exists_Psi9}, we know $ \epsilon$ is monotonically increasing for $\alpha>0$ and when $0<\alpha<\zeta_1$, we have $0<\epsilon <1$.

\begin{lemma} \label{lemma:bound_consensus_jointly} 
    Suppose that Assumptions~\ref{assum:weighted matrix} and \ref{assum:A and b} hold and $\{ \bbb{G}_t \}$ is uniformly strongly connected by sub-sequences of length $L$. Then, when $\alpha \in (0, \zeta_1)$, we have for all $t \ge \tau(\alpha)$, 
$$
    \sum_{i=1}^N \pi_{t}^i \| \theta_{t}^i - \langle \theta \rangle_{t} \|_2^2 \le \epsilon^{q_{t}} \sum_{i=1}^N \pi_{m_t}^i \| \theta_{m_t}^i - \langle \theta \rangle_{m_t} \|_2^2 + \frac{\zeta_2}{1- \epsilon},
$$
where $\zeta_1$ is defined in Appendix~\ref{sec:constants}, $ \epsilon$ and $\zeta_2$ are defined in \eqref{eq:define epsilon_jointly} and \eqref{eq:define Psi10}, respectively.
\end{lemma}









\begin{lemma} \label{lemma:bound_average}
    Suppose that Assumptions~\ref{assum:A and b}--\ref{assum:lyapunov} and \ref{assum:limit_pi} hold. Then, when 
    $
    0< \alpha < \min\{\frac{ \log2}{A_{\max} \tau(\alpha)},\; \frac{0.1}{K_2 \gamma_{\max}}\},
$
    we have for any $t \ge T_1$,
%\begin{align*}
%    %\mathbf{E}[ \| \langle \Theta_{t+1} \rangle_{t+1}^\top - \theta^* \|_2^2] \le (1-\sigma_{\min} \alpha)^{t+1-\tau(\alpha)} \left(10 \mathbf{E}[\|  \langle \Theta_{0} \rangle_{0}^\top - \theta^*\|_2^2] + 8( \| \theta^*\|_2^2 +R)^2]  \right) + \frac{\zeta_3 \alpha}{\sigma_{\min}},
%    \mathbf{E}\left[ \| \langle \theta \rangle_{t+1} - \theta^* \|_2^2\right] 
%    & \le \left(1 - \frac{0.9  \alpha}{\gamma_{\max}} \right)^{t+1-T_1^*}  \frac{\gamma_{\max}}{\gamma_{\min}} \mathbf{E}\left[ \| \langle \theta \rangle_{T_1^*} - \theta^* \|_2^2 \right] +  \frac{\gamma_{\max}}{\gamma_{\min}}\cdot \frac{\alpha  \zeta_3 \gamma_{\max} + 2  \gamma_{\max}  \zeta_4}{0.9  }  \\
%    & \le \left(1 - \frac{0.9  \alpha}{\gamma_{\max}} \right)^{t+1-T_1^*} \frac{\gamma_{\max}}{\gamma_{\min}} \left( 4 \exp\left\{ 2 \alpha A_{\max}T_1^* \right\}+2\right)  \mathbf{E}\left[\|\langle \theta \rangle_{0} -\theta^* \|_2^2\right] \nonumber\\
%    &\;\;\; + 4 \left(1 - \frac{0.9  \alpha}{\gamma_{\max}} \right)^{t+1-T_1^*} \frac{\gamma_{\max}}{\gamma_{\min}} \exp\left\{ 2\alpha A_{\max}T_1^* \right\} \left( \|\theta^*\|_2 + \frac{b_{\max}}{A_{\max}} \right)^2 \\
%    & \;\;\; +  \frac{\gamma_{\max}}{\gamma_{\min}}\cdot \frac{\alpha  \zeta_3 \gamma_{\max} + 2  \gamma_{\max}  \zeta_4}{0.9  }, 
%\end{align*}
%{\color{red}
%\begin{align*}
%    \mathbf{E}\left[ \| \langle \theta \rangle_{t} - \theta^* \|_2^2\right] 
%    & \le \left(1 - \frac{0.9  \alpha}{\gamma_{\max}} \right)^{t-T_1}  \frac{\gamma_{\max}}{\gamma_{\min}} \mathbf{E}\left[ \| \langle \theta \rangle_{T_1} - \theta^* \|_2^2 \right] +  \frac{\gamma_{\max}}{\gamma_{\min}}\cdot \frac{\alpha  \zeta_3 \gamma_{\max} + 2  \gamma_{\max}  \zeta_4}{0.9  }  \\
%    & \le \left(1 - \frac{0.9  \alpha}{\gamma_{\max}} \right)^{t-T_1} \frac{\gamma_{\max}}{\gamma_{\min}} \left( 4 \exp\left\{ 2 \alpha A_{\max}T_1 \right\}+2\right)  \mathbf{E}\left[\|\langle \theta \rangle_{0} -\theta^* \|_2^2\right] \nonumber\\
%    &\;\;\; + 4 \left(1 - \frac{0.9  \alpha}{\gamma_{\max}} \right)^{t-T_1} \frac{\gamma_{\max}}{\gamma_{\min}} \exp\left\{ 2\alpha A_{\max}T_1 \right\} \left( \|\theta^*\|_2 + \frac{b_{\max}}{A_{\max}} \right)^2 \\
%    & \;\;\; +  \frac{\gamma_{\max}}{\gamma_{\min}}\cdot \frac{\alpha  \zeta_3 \gamma_{\max} + 2  \gamma_{\max}  \zeta_4}{0.9  }, 
%\end{align*}
%===========================
\begin{align*}
    &\;\;\;\; \mathbf{E}[\|\langle \theta \rangle_{t+1} -\theta^* \|_2^2 ] \\
    & \le \Big(1 - \frac{0.9  \alpha}{\gamma_{\max}} \Big)^{t-T_1}  \frac{\gamma_{\max}}{\gamma_{\min}} \mathbf{E}\left[ \| \langle \theta \rangle_{T_1} - \theta^* \|_2^2 \right] +  \frac{\alpha  \zeta_3 \gamma_{\max}^2}{0.9 \gamma_{\min} }  \\
    &\;\;\; + \frac{\gamma_{\max}}{\gamma_{\min}} \alpha \zeta_4 \sum_{k={0}}^{t-T_1}  \eta_{t+1-k}  \Big(1-\frac{0.9  \alpha}{\gamma_{\max}} \Big)^{k}  \\
    & \le \Big(1 - \frac{0.9  \alpha}{\gamma_{\max}} \Big)^{t+1-T_1} \frac{C_1}{2}  +  \frac{\alpha  \zeta_3 \gamma_{\max}^2}{0.9 \gamma_{\min} }\\
    %& \le \Big(1 - \frac{0.9  \alpha}{\gamma_{\max}} \Big)^{t+1-T_1} \frac{C_1}{2} \frac{\gamma_{\max}}{\gamma_{\min}} ( 4 \exp\left\{ 2 \alpha A_{\max}T_1 \right\}+2)  \mathbf{E}[\|\langle \theta \rangle_{0} -\theta^* \|_2^2] \nonumber\\
    %& + 4 \Big(1 - \frac{0.9  \alpha}{\gamma_{\max}} \Big)^{t+1-T_1} \frac{\gamma_{\max}}{\gamma_{\min}} \exp\left\{ 2\alpha A_{\max}T_1 \right\} \Big( \|\theta^*\|_2 + \frac{b_{\max}}{A_{\max}} \Big)^2 \\
    &\;\;\;  + \frac{\gamma_{\max}}{\gamma_{\min}} \alpha \zeta_4 \sum_{k={0}}^{t-T_1}  \eta_{t+1-k}  \Big(1-\frac{0.9  \alpha}{\gamma_{\max}} \Big)^{k} . 
\end{align*}
where $C_1$, $\zeta_3$, $\zeta_4$ and $K_2$ are defined in Appendix~\ref{sec:thmSA_constant}, \eqref{eq:define Psi4}, \eqref{eq:define Psi5} and \eqref{eq:define Psi3}, respectively.
\end{lemma}


We are now in a position to prove the fixed step-size case in Theorem~\ref{thm:bound_jointly_SA}.

%\vspace{.1in}

\noindent
{\bf Proof of Case 1) in Theorem~\ref{thm:bound_jointly_SA}:}
%{\color{red}
%Note that Lemma~\ref{lemma:bound_average} still holds when $\{\bbb{G}_t\}$ is uniformly strongly connected.
%Using the same argument as in the proof of Lemma~\ref{lemma:bound_average}, the lemma still holds here when $T^*_1$ is replaced by $T^*_3$. 
%} 
From Lemmas~\ref{lemma:bound_consensus_jointly} and \ref{lemma:bound_average}, we have for any $t \ge T_1$,
%\begin{align*}
%        & \;\;\;\; \sum_{i=1}^N \pi_{t}^i \mathbf{E}[\|\theta_{t}^i - \theta^*\|_2^2] \nonumber\\
%        & \le 2 \sum_{i=1}^N \pi_{t}^i \mathbf{E}[\|\theta_{t}^i - \langle \theta \rangle_{t} \|_2^2 ] + 2 \mathbf{E} [\| \langle \theta \rangle_{t} - \theta^*\|_2^2] \\
%        &\le 2  \epsilon^{q_{t}} \sum_{i=1}^N \pi_{m_t}^i \mathbf{E}[\| \theta_{m_t}^i - \langle \theta \rangle_{m_t} \|_2^2] + \frac{2 \zeta_2}{1- \epsilon} + \frac{\gamma_{\max}}{\gamma_{\min}}\cdot \frac{ 2 \alpha  \zeta_3 \gamma_{\max} + 4 \gamma_{\max}  \zeta_4}{0.9  }  \nonumber\\
%        &\;\;\; + \left(1 - \frac{0.9  \alpha}{\gamma_{\max}} \right)^{{t}-T_1}\frac{\gamma_{\max}}{\gamma_{\min}} ( 8 \exp\left\{ 2 \alpha A_{\max}T_1 \right\}+4)  \mathbf{E}[\| \langle \theta \rangle_{0} -\theta^* \|_2^2] \nonumber\\
%        &\;\;\; + 8 \left(1 - \frac{0.9  \alpha}{\gamma_{\max}} \right)^{{t}-T_1} \frac{\gamma_{\max}}{\gamma_{\min}} \exp\left\{ 2\alpha A_{\max}T_1 \right\} ( \|\theta^*\|_2 + \frac{b_{\max}}{A_{\max}} )^2 \\
%        &\le 2 \epsilon^{q_{t}} \sum_{i=1}^N \pi_{m_t}^i \mathbf{E}\left[\left\| \theta_{m_t}^i - \langle \theta \rangle_{m_t} \right\|_2^2 \right]  + C_1 \bigg( 1 - \frac{0.9  \alpha}{\gamma_{\max}} \bigg)^{{t}-T_1}  + C_2,
%\end{align*}
\begin{align*}
        &\;\;\;\; \sum_{i=1}^N \pi_{t}^i \mathbf{E}[\|\theta_{t}^i - \theta^*\|_2^2] \\
        &\le 2 \sum_{i=1}^N \pi_{t}^i \mathbf{E}[\|\theta_{t}^i - \langle \theta \rangle_{t} \|_2^2 ] + 2 \mathbf{E} [\| \langle \theta \rangle_{t} - \theta^*\|_2^2] \\
        &\le 2  \epsilon^{q_{t}} \sum_{i=1}^N \pi_{m_t}^i \mathbf{E}[\| \theta_{m_t}^i - \langle \theta \rangle_{m_t} \|_2^2]  \\
        &\;\;\; + \frac{2 \zeta_2}{1- \epsilon} +  \frac{2 \alpha  \zeta_3 \gamma_{\max}^2}{0.9 \gamma_{\min} } + \Big(1 - \frac{0.9  \alpha}{\gamma_{\max}} \Big)^{{t}-T_1}C_1\\
        &\;\;\; + \frac{\gamma_{\max}}{\gamma_{\min}} 2\alpha \zeta_4 \sum_{k={0}}^{t-T_1}  \eta_{t+1-k}  \Big(1-\frac{0.9  \alpha}{\gamma_{\max}} \Big)^{k}    \\
        %&\;\;\; + \Big(1 - \frac{0.9  \alpha}{\gamma_{\max}} \Big)^{{t}-T_1}\frac{\gamma_{\max}}{\gamma_{\min}} ( 8 \exp\left\{ 2 \alpha A_{\max}T_1 \right\}+4)  \mathbf{E}[\| \langle \theta \rangle_{0} -\theta^* \|_2^2] \nonumber\\
        %&\;\;\; + 8 \Big(1 - \frac{0.9  \alpha}{\gamma_{\max}} \Big)^{{t}-T_1} \frac{\gamma_{\max}}{\gamma_{\min}} \exp\left\{ 2\alpha A_{\max}T_1 \right\} \Big( \|\theta^*\|_2 + \frac{b_{\max}}{A_{\max}} \Big)^2 \\
        &\le 2 \epsilon^{q_{t}} \sum_{i=1}^N \pi_{m_t}^i \mathbf{E}[\| \theta_{m_t}^i - \langle \theta \rangle_{m_t} \|_2^2 ]  + C_1 \Big( 1 - \frac{0.9  \alpha}{\gamma_{\max}} \Big)^{{t}-T_1}\\
        &\;\;\; + C_2 + \frac{\gamma_{\max}}{\gamma_{\min}} 2\alpha \zeta_4 \sum_{k={0}}^{t-T_1}  \eta_{t+1-k}  \Big(1-\frac{0.9  \alpha}{\gamma_{\max}} \Big)^{k},
\end{align*}
where $C_1$ and $C_2$ are defined in Appendix~\ref{sec:thmSA_constant}.
This completes the proof.
\hfill $\qed$



%{\color{blue} Note that, we have $\lim_{t\to\infty} \sum_{k=0}^{t-T_1} \eta_{t+1-k} (1-\frac{0.9 \alpha}{\gamma_{\max}})^k \le \lim_{t\to\infty} \frac{\gamma_{\max}}{0.9 \alpha} [ \eta_{\ceil{\frac{t+1}{2}}} + \eta_1 (1-\frac{0.9 \alpha}{\gamma_{\max}})^{\frac{t}{2}} ] = 0 $}

\subsubsection{Time-varying Step-size} \label{sec:proof_jointly_time-varying}

In this subsection, we consider the time-varying step-size case and begin with a property of $\eta_t$.


\begin{lemma} \label{lemma:eta_sum}
    Suppose that Assumption~\ref{assum:limit_pi} holds. Then, $\lim_{t \to \infty} \eta_t =0$ and $\lim_{t \to \infty} \frac{1}{t+1} \sum_{k=0}^t \eta_{k} = 0.$
\end{lemma}



%Recall the updates corresponding to the time-varying step-size case given in


To prove the theorem, we need the following lemmas.



\begin{lemma} \label{lemma:bound_consensus_time-varying_jointly} 
Suppose that Assumptions~\ref{assum:weighted matrix} and \ref{assum:A and b} hold and $\{ \bbb{G}_t \}$ is uniformly strongly connected by sub-sequences of length $L$. 
%    Let $q_t$ and $m_t$ be the unique integer quotient and remainder of $t$ divided by $L$, respectively.
    Given $\alpha_t$ and $T_2$ defined in Theorem~\ref{thm:bound_jointly_SA}, for all $t \ge T_2L $,
    \begin{align*} 
        &\sum_{i=1}^N \pi_{t}^i \| \theta_{t}^i - \langle \theta \rangle_{t} \|_2^2 
        \le \frac{\zeta_6}{1-\epsilon} \left(  \epsilon^{\frac{q_t - 1}{2}}  \alpha_{m_t} + \alpha_{\ceil{\frac{q_t - 1}{2}} L+m_t} \right) \\
        &\;\;\;\;\;\; +  \epsilon^{q_{t}-{T_2}}  \sum_{i=1}^N \pi_{T_2L + m_t }^i \| \theta_{T_2L + m_t }^i - \langle \theta \rangle_{T_2L+ m_t } \|_2^2,
    \end{align*}
    which implies that 
    \begin{align*} 
        & \sum_{i=1}^N \pi_{t}^i \| \theta_{t}^i - \langle \theta \rangle_{t} \|_2^2 
        \le \frac{\zeta_6}{1-\epsilon} \left( \alpha_0 \epsilon^{\frac{q_t-1}{2}} + \alpha_{\ceil{\frac{q_t-1}{2}}L} \right)   \\
        &\;\;\;\;\;\;\; + \epsilon^{q_t - {T_2}} \sum_{i=1}^N \pi_{T_2L+m_t}^i \| \theta_{T_2L+m_t}^i - \langle \theta \rangle_{T_2L+m_t} \|_2^2,
    \end{align*}
where $\epsilon$ and $\zeta_6$ are defined in \eqref{eq:define epsilon_jointly} and \eqref{eq:define Psi11}, respectively.
\end{lemma}



%{\color{blue}
%\begin{lemma} \label{lemma:bound_consensus_time-varying_jointly_allt} 
%    Suppose that Assumptions~\ref{assum:weighted matrix} and \ref{assum:A and b} hold and $\{ \bbb{G}_t \}$ is uniformly strongly connected by sub-sequences of length $L$. 
%    Let $q_t$ and $m_t$ be the unique integer quotient and remainder of $t$ divided by $L$, respectively.
%    Given $\alpha_t$ and $T_2$ defined in Theorem~\ref{thm:bound_time-varying_step}, for all $t \ge T_2L $,
%    \begin{align*} 
%        \sum_{i=1}^N \pi_{t}^i \| \theta_{t}^i - \langle \theta \rangle_{t} \|_2^2
%        & \le \hat \epsilon^{q_{t}-{T_2}}  \sum_{i=1}^N \pi_{T_2L + m_t }^i \| \theta_{T_2L + m_t }^i - \langle \theta \rangle_{T_2L+ m_t } \|_2^2 + \frac{\zeta_6}{1-\hat\epsilon} \left(  \hat\epsilon^{\frac{q_t - 1}{2}}  \alpha_{m_t} + \alpha_{\ceil{\frac{q_t - 1}{2}} L+m_t} \right) \\
%        & \le \hat \epsilon^{q_t - {T_2}} \sum_{i=1}^N \pi_{T_2L+m_t}^i \| \theta_{T_2L+m_t}^i - \langle \theta \rangle_{T_2L+m_t} \|_2^2 + \frac{\zeta_6}{1-\hat\epsilon} \left( \alpha_0 \hat\epsilon^{\frac{q_t-1}{2}} + \alpha_{\ceil{\frac{q_t-1}{2}}L} \right),
%    \end{align*}
%where $\hat\epsilon$ and $\zeta_6$ is defined in \eqref{eq:define epsilon_jointly} and \eqref{eq:define Psi11}, respectively.
%\end{lemma}}















\begin{lemma} \label{lemma:bound_average_time-varying_jointly}
    Under Assumptions~\ref{assum:weighted matrix}--\ref{assum:limit_pi}, when the $$\tau(\alpha_t) \alpha_{t-\tau(\alpha_t)} \le \min \{ \frac{ \log2}{A_{\max}}, \; \frac{0.1}{\zeta_5 \gamma_{\max}} \},$$ we have for any $t\ge T_2L$,
%    \begin{align*}
%        \mathbf{E}[\| \langle \theta \rangle_{t+1} -\theta^* \|_2^2 ] 
%        & \le \frac{T_2L}{t+1} \frac{\gamma_{\max}}{\gamma_{\min}} \mathbf{E}[\| \langle \theta \rangle_{T_2L} -\theta^* \|_2^2 ] 
%        +  \frac{\zeta_7 \alpha_0  C \log^2(\frac{t+1}{\alpha_0})}{t+1} \frac{\gamma_{\max}}{\gamma_{\min}}
%     \nonumber\\
%        & \;\;\; +  \alpha_0 \zeta_4 \frac{\gamma_{\max}}{\gamma_{\min}}  \frac{\sum_{l = T_2L}^{t} \eta_{l+1}}{t+1}.
%    \end{align*}
\begin{align*}
    &\;\;\;\; \mathbf{E} \left[\|\langle \theta \rangle_{t} -\theta^* \|_2^2 \right] \le \frac{T_2L}{t} \frac{\gamma_{\max}}{\gamma_{\min}} \mathbf{E}[\| \langle \theta \rangle_{T_2L} -\theta^* \|_2^2 ] \\
    &
    +  \frac{\zeta_7 \alpha_0  C \log^2(\frac{t}{\alpha_0})}{t} \frac{\gamma_{\max}}{\gamma_{\min}}  +  \alpha_0 \zeta_4 \frac{\gamma_{\max}}{\gamma_{\min}}  \frac{\sum_{l = T_2L}^{t} \eta_{l}}{t},
\end{align*}
where $T_2$ is defined in Appendix~\ref{sec:thmSA_constant}, and $\zeta_4$, $\zeta_5$, $\zeta_7$ are defined in \eqref{eq:define Psi5}, \eqref{eq:define Psi7}, \eqref{eq:define Psi8}, respectively.
\end{lemma}



We are now in a position to prove the time-varying step-size case in  Theorem~\ref{thm:bound_jointly_SA}.

\noindent
{\bf Proof of Case 2) in Theorem~\ref{thm:bound_jointly_SA}:}
From Lemmas~\ref{lemma:bound_consensus_time-varying_jointly} and \ref{lemma:bound_average_time-varying_jointly}, for any $t \ge T_2L$, we have
    \begin{align*}
        & \;\;\;\; \sum_{i=1}^N \pi_{t}^i \mathbf{E}[\|\theta_{t}^i - \theta^*\|_2^2] \\
        & \le 2 \sum_{i=1}^N \pi_{t}^i \mathbf{E}[\|\theta_{t}^i - \langle \theta \rangle_{t} \|_2^2 ] + 2 \mathbf{E} [\| \langle \theta \rangle_{t} - \theta^*\|_2^2]\\
        & \le 2  \epsilon^{q_{t}-{T_2}} \sum_{i=1}^N \pi_{T_2L+m_t}^i \mathbf{E}[\| \theta_{T_2L+m_t}^i - \langle \theta \rangle_{T_2L+m_t} \|_2^2]  \\
        &+ \frac{2T_2L}{t} \frac{\gamma_{\max}}{\gamma_{\min}} \mathbf{E}[\| \langle \theta \rangle_{T_2L} -\theta^* \|_2^2 ] +  2 \alpha_0 \zeta_4 \frac{\gamma_{\max}}{\gamma_{\min}} \frac{\sum_{l = T_2L}^{t} \eta_{l}}{t} \\
        &
        +  \frac{2\zeta_7 \alpha_0  C \log^2(\frac{t}{\alpha_0})}{t} \frac{\gamma_{\max}}{\gamma_{\min}}
         + \frac{2\zeta_6}{1-\epsilon} ( \alpha_0 \epsilon^{\frac{q_t-1}{2}} + \alpha_{\ceil{\frac{q_t-1}{2}}L}) \\
        & \le  2  \epsilon^{q_{t}-T_2} \sum_{i=1}^N \pi_{LT_2+m_t}^i \mathbf{E}\left[\left\| \theta_{LT_2+m_t}^i - \langle \theta \rangle_{LT_2+m_t} \right\|_2^2\right] \\
        &+ C_3 \left( \alpha_0  \epsilon^{\frac{q_t-1}{2}} + \alpha_{\ceil{\frac{q_t-1}{2}}L}\right) \nonumber  \\
        &+  \frac{1}{t} \bigg(C_4 \log^2\Big(\frac{t}{\alpha_0}\Big)+C_5\sum_{k = LT_2}^{t} \eta_{k} + C_6\bigg),
    \end{align*}
    where $C_3 - C_6$ are defined in Appendix~\ref{sec:thmSA_constant}.
    This completes the proof.
\hfill $\qed$


{\color{black}
\begin{remark}
For distributed SA algorithms, finite-time performance analysis essentially boils down to two parts, namely bounding the consensus error and bounding the ``single-agent’’ mean-square error. For the case when consensus interaction matrices are all doubly stochastic, the consensus error bound can be derived by analyzing the square of the 2-norm of the deviation of the current state of each agent from the average of the states of the agents. With consensus in the presence of doubly stochastic matrices, the average of the states of the agents remains invariant. Thus, it is possible to treat the average value as the state of a fictitious agent to derive the mean-square consensus error bound with respect to the limiting point. More formally, this process relies on two properties of a doubly stochastic matrix $W$, namely that (1) $\1^\top W =\1^\top$, and (2) if $x_{t+1}=Wx_t$, then $\|x_{t+1} - (\1^\top x_{t+1})\1\|_2 \le \sigma_2(W) \|x_{t} - (\1^\top x_{t})\1\|_2$ where $\sigma_2(W)$ denotes the second largest singular value of $W$ (which is strictly less than one if $W$ is irreducible). Even if the doubly stochastic matrix is time-varying (denoted by $W_t$), property (1) still holds and property (2) can be generalized as in \cite{nedic2018network}. Thus, the square of the 2-norm $\|x_{t} - (\1^\top x_{t})\1\|_2^2$ is a quadratic Lyapunov function for the average consensus processes. Doubly stochastic matrices in expectation can be treated in the same way by looking at the expectation. 
This is the core on which all the existing finite-time analyses of distributed RL algorithms are based. However, if each consensus interaction matrix is stochastic, and not necessarily doubly stochastic, the above two properties may not hold. In fact, it is well known that quadratic Lyapunov functions for general consensus processes $x_{t+1}=S_tx_t$, with $S_t$ being stochastic, do not exist \cite{olshevsky2008nonexistence}. Here we appeal to the idea of quadratic comparison functions for general consensus processes. This was first proposed in \cite{touri2012product} and makes use of the concept of absolute probability sequences. 
We provide a general analysis methodology and results that subsume the existing finite-time analyses for single-timescale distributed linear stochastic approximation (Lemmas~\ref{lemma:bound_consensus_jointly}, \ref{lemma:bound_average}, \ref{lemma:bound_consensus_time-varying_jointly} and \ref{lemma:bound_average_time-varying_jointly}) and TD learning as special cases. 
\hfill$\Box$
\end{remark}
}




%{\color{cyan}Note that, we can use Lemmas~\ref{lemma:bound_consensus_jointly}, \ref{lemma:bound_average}, \ref{lemma:bound_consensus_time-varying_jointly} and \ref{lemma:bound_average_time-varying_jointly} to obtain the bounds for fixed step-size and time-varying step-size in Theorem~\ref{thm:bound_jointly_SA}, respectively. Besides, Lemmas~\ref{lemma:ration_in_0_1} and \ref{lemma:eta_sum} guarantee the convergence of the bounds in Theorem~\ref{thm:bound_jointly_SA}.}

==> Proof_push.tex <==


Let $\hat W_t$ be the matrix whose $ij$-th entry is $\hat w_t^{ij}$. Then, from \eqref{eq:SA_push-sum} we have
\begin{align}
    &\theta^i_{t+1}=\frac{\tilde \theta^i_{t+1}}{y^i_{t+1}} = \frac{\sum_{j=1}^N \hat w_t^{ij } ( \tilde \theta^j_{t} + \alpha_t A(X_t) \theta^j_{t} + \alpha_t b^j(X_t ))} {y^i_{t+1}} \nonumber \\
    &= \sum_{j=1}^N \frac{\hat w_t^{ij} y_t^j}{\sum_{k=1}^N \hat w_t^{ik } y^k_{t}} \left[ \frac{\tilde \theta^j_{t}}{y_t^j} + \alpha_t A(X_t) \frac{ \theta^j_{t}}{y_t^j} + \alpha_t \frac{ b^j(X_t ) }{y_t^j}\right]  \nonumber \\
    &= \sum_{j=1}^N \tilde w_t^{ij}  \left[ \theta^j_{t} + \alpha_t A(X_t) \frac{ \theta^j_{t}}{y_t^j} + \alpha_t \frac{ b^j(X_t ) }{y_t^j}\right], \label{eq:push-sum_ratio}
\end{align}
where $ \tilde w_t^{ij} = \frac{\hat w_t^{ij} y_t^j}{\sum_{k=1}^N \hat w_t^{ik } y^k_{t}}$ and $ \tilde W_t = [ \tilde w_t^{ij}]$ is a row stochastic matrix, i.e.,
$
    \sum_{j=1}^N \tilde w_t^{ij} = \frac{\sum_{j=1}^N \hat w_t^{ij} y_t^j}{\sum_{k=1}^N \hat w_t^{ik } y^k_{t}} =1,
$
for all $i$.



Let $\Theta_t = [\theta_t^1, \cdots, \theta_t^N]^\top$ 
%and $\tilde \Theta_t = [\tilde \theta_t^1, \cdots, \tilde \theta_t^N]^\top$
. Then %\eqref{eq:SA_push-sum} and 
\eqref{eq:push-sum_ratio} can be written as
\begin{align}
    \Theta_{t+1} &=  \tilde W_t \Bigg[\Theta_{t} + \alpha_t 
    \left[
    \begin{array}{c}
        ( \theta_t^1)^\top/ y_t^1 \\
        \cdots \\
        ( \theta_t^N)^\top / y_t^N
    \end{array}
    \right] A(X_t)^\top
    \nonumber\\
    &\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; + \alpha_t
    \left[
    \begin{array}{c}
        (b^1(X_t))^\top / y_t^1 \\
        \cdots \\
        (b^N(X_t))^\top / y_t^N
    \end{array}
    \right]
    \Bigg]. \label{eq:update Theta}
\end{align}
%\begin{align}
%    \tilde\Theta_{t+1} &= (\tilde W_t \otimes I_K) \left[\tilde\Theta_{t} + \alpha_t 
%    \left[
%    \begin{array}{c}
%        A(X_t) \tilde \theta_t^1/ y_t^1 \\
%        \cdots \\
%        A(X_t) \tilde \theta_t^N/ y_t^N
%    \end{array}
%    \right]
%    + \alpha_t B(X_t) \right] \\
%    \Theta_{t+1} &= ( W_t \otimes I_K) \left[\Theta_{t} + \alpha_t 
%    \left[
%    \begin{array}{c}
%        A(X_t)  \theta_t^1/ y_t^1 \\
%        \cdots \\
%        A(X_t)  \theta_t^N/ y_t^N
%    \end{array}
%    \right]
%    + \alpha_t
%    \left[
%    \begin{array}{c}
%        b^1(X_t) / y_t^1 \\
%        \cdots \\
%        b^N(X_t) / y_t^N
%    \end{array}
%    \right]
%    \right] \label{eq:update Theta}
%\end{align}
%where $B(X_t) = [(b^1(X_t))^\top \cdots (b^N(X_t))^\top]^\top$.

%\subsubsection{The Boundness}
%{\color{red} Our main goal is to find a constant $C$ such that $ \| \theta_n^i - \frac{\sum_{j=1}^N \tilde \theta_n^j}{N} \| \le C $ for all $n$. }


%\subsection{Kaiqing and Borkar's idea}


Since each matrix $\tilde W_t = [\tilde w_t^{ij}]$ is stochastic, from Lemma~\ref{lemma:bound_pi_jointly}, there exists a unique absolute  probability  sequence $\{ \tilde \pi_t \} $ for  the  matrix  sequence $\{ \tilde W_t \} $ such that $ \tilde \pi_t^i \ge \tilde  \pi_{\min}$ for all $i\in\mathcal V$ and $t\ge 0$, with the constant $ \tilde \pi_{\min}\in(0,1)$.

\begin{lemma} \label{lemma:pushsum_product}
    Suppose that $\{ \bbb{G}_t \}$ is uniformly strongly connected. Then, $\Pi_{s=0}^t \hat W_s $ will converge to the set $\{v\1_N^\top \; :\; v\in\R^N\}$ exponentially fast as $t\rightarrow\infty$.
\end{lemma}



\begin{lemma} \label{lemma:push-sum_pi_intfty}
    Suppose that $\{ \bbb{G}_t \}$ is uniformly strongly connected. Then,
    $ (\Pi_{l=s}^{t} \tilde W_l)^{ij}= \frac{y_s^j}{y_{t+1}^i} (\Pi_{l=s}^{t} \hat W_l)^{ij} $  and $\frac{\tilde \pi_s^i}{y_s^i} = \frac{1}{y_s^i}\lim_{t\to\infty} (\Pi_{l=s}^{t} \tilde W_l)^{ji} = \frac{1}{N}$ for all $i,j\in\mathcal V$ and $s \ge 0$.
\end{lemma}


%{\color{blue}
%By using the properties proposed in Lemma~\ref{lemma:push-sum_pi_intfty}, we can obtain the following lemma. }





\begin{lemma} \label{lemma:bound_theta}
The sequence $\{ \Theta_n \}$ generated by \eqref{eq:update Theta} is bounded almost surely, i.e., $ C_\theta = \sup_{n} \| \Theta_n \|_F<\infty$ almost surely.
\end{lemma}



From \eqref{eq:SA_push-sum},
%\begin{align*}
%    \tilde \theta^i_{t+1} &= \sum_{j =1}^N  \hat w_t^{ij } \left[ \tilde\theta^j_{t}  + \alpha_t \left(A(X_{t}) \theta^j_{t} + b^j(X_{t} ) \right) \right].
%\end{align*}
by using the definition of $\langle \tilde \theta \rangle_t = \frac{1}{N} \sum_{i=1}^N \tilde \theta_t^i$ and $\langle \theta \rangle_t = \frac{1}{N} \sum_{i=1}^N \theta_t^i$, we have
\begin{align} \label{eq:update_average_tilde_theta}
    &\;\;\;\; \langle \tilde \theta \rangle_{t+1}
    = \langle \tilde \theta \rangle_t + \alpha_t A(X_t) \langle \theta \rangle_t + \frac{\alpha_t}{N}\sum_{i=1}^N b^i(X_t) \nonumber \\
    &= \langle \tilde \theta\rangle_t  + \alpha_t A(X_t) \langle \tilde \theta \rangle_t + \frac{\alpha_t}{N}\sum_{i=1}^N b^i(X_t)  +   \alpha_t \rho_t,
\end{align}
where $ \rho_t = A(X_t) \langle \theta \rangle_t - A(X_t) \langle \tilde \theta \rangle_t$. From Lemma~\ref{lemma:bound_theta}, we have $\| \langle \theta \rangle_t \|_2 \le \max_{i\in\mathcal{V}} \| \theta_t^i \|_2 \le C_\theta$ for all $t \ge 0$, which implies that $\| \langle \tilde \theta \rangle_t \|_2 \le N C_\theta$ and
$
    \mu_t = \| \rho_t \|_2 = \left\| A(X_t) \langle \theta \rangle_t - A(X_t) \langle \tilde \theta  \rangle_t \right\|_2 \le \mu_{\max},
$
where $\mu_{\max} = (N+1) A_{\max} C_\theta$.




%\begin{theorem} %\label{thm:bound_time-varying_step_Push_SA}
%    {\color{red}
%    Suppose that Assumptions~\ref{assum:A and b}--\ref{assum:lyapunov}
%    hold and $\{ \bbb{G}_t \}$ is uniformly strongly connected by sub-sequences of length $L$. 
%    Let $\{ \theta_t^i \}$, $i\in \mathcal{V}$, be generated by \eqref{eq:push-sum_ratio}
%    with $\alpha_t = \frac{\alpha_0}{t+1}$ and $\alpha_0 \ge \frac{\gamma_{\max}}{0.9}$. 
    %Let $\alpha$ be any constant satisfying $0 < \alpha < \min \left\{ \frac{\log2}{A_{\max} \tau(\alpha)},\; \frac{0.1}{\Psi_1 \gamma_{\max}}\right\}$, where $\Psi_3$ is given in \eqref{eq:define Psi3}.
%    Let $\epsilon_1 > 0$ and $\bar\epsilon \in (0,1)$ satisfy $\epsilon_1 \ge \frac{1}{N^{NL}}$ and $\bar\epsilon \le (1-\frac{1}{N^{NL}})^{1/L}$.
%    Define the constants $\Psi_{1}$ and $\Psi_{2}$ as
%    \begin{align}
%    \Psi_1 &= 2 \left( 72 + 458 A_{\max}^2  + 84  A_{\max}  b_{\max} + 72 A_{\max} \mu_{\max} \right) \label{eq:definition_Psi1}\\
%    \Psi_2 &= \bigg[ 2 + ( 4 + \Psi_1) \|\theta^* \|_2^2 +  48\frac{(b_{\max}+ \mu_{\max})^2}{A_{\max}^2} +  152  \left(b_{\max} + \mu_{\max} + A_{\max} \| \theta^* \|_2 \right)^2  \nonumber\\
%    &\;\;\;\; +  12  A_{\max}b_{\max} + 48  A_{\max}(b_{\max}+ \mu_{\max}) (\frac{b_{\max} + \mu_{\max}}{A_{\max}} + 1 )^2 +  89 (b_{\max}+ \mu_{\max})^2  \bigg]\label{eq:definition_Psi2}
%\end{align}
    %Let $\bar T$ be any positive integer such that for all $t\ge \bar T$, there hold $2\tau(\alpha_t) \le t$, $\| \mu_{t} \|_2 \le \frac{0.05}{\gamma_{\max}}$ and $\tau(\alpha_t) \alpha_{t-\tau(\alpha_t)} \le \min \{ \frac{ \log2}{A_{\max}},\; \frac{0.05}{\Psi_1 \gamma_{\max}} \}$. 
%    Let $\bar T$ be any positive integer such that for all $t\ge \bar T$, there hold $2\tau(\alpha_t) \le t$, $\| \mu_{t} \|_2 + \tau(\alpha_t) \alpha_{t-\tau(\alpha_t)} \Psi_1 \le \frac{0.1}{\gamma_{\max}}$ and $\tau(\alpha_t) \alpha_{t-\tau(\alpha_t)} \le \min \{ \frac{ \log2}{A_{\max}},\; \frac{0.1}{\Psi_1 \gamma_{\max}} \}$. 
%    Then, for all $t\ge \bar T$,}
%    \begin{align*}
%        \sum_{i=1}^N \mathbf{E}[\|\theta_{t+1}^i - \theta^*\|_2^2] 
%        & \le \frac{16}{\epsilon_1}  \bar\epsilon^t \mathbf{E}[ \| \sum_{i=1}^N \tilde \theta_0^i + \alpha_0 A(X_0)\theta_0^i + \alpha_0 b^i(X_0) \|_2] + \frac{16}{\epsilon_1} \frac{ A_{\max} C_\theta + b_{\max}}{1-\bar\epsilon} \left(  \alpha_0 \bar\epsilon^{t/2}  +  \alpha_{\ceil{\frac{t}{2}}} \right) \\
%        & \;\;\; + 2 \alpha_t  A_{\max} C_\theta + 2 \alpha_t b_{\max} + \frac{2\bar TN}{t} \frac{\gamma_{\max}}{\gamma_{\min}} \mathbf{E}[\|\langle \tilde \theta\rangle_{\bar T}  -\theta^* \|_2^2 ] \\
%        &\;\;\; 
%        +  \frac{2 N \Psi_2 \alpha_0  C \log^2(\frac{t}{\alpha_0})}{t} \frac{\gamma_{\max}}{\gamma_{\min}}
%        +  2 \alpha_0 N \frac{\gamma_{\max}}{\gamma_{\min}} \frac{\sum_{l = \bar T}^{t} \| \mu_{l} \|_2 }{t}
%    \end{align*}
    %\begin{align*}
    %    \sum_{i=1}^N \mathbf{E}[\|\theta_{t+1}^i - \theta^*\|_2^2] 
    %    & \le \frac{16N}{\epsilon_1}  \bar\epsilon^t \mathbf{E}[ \| \tilde \Theta_0 \|_1] + \frac{16}{\epsilon_1} \frac{N^2 \sqrt{K} (A_{\max} C_\theta + b_{\max})}{1-\bar\epsilon} \left(  \alpha_0 \bar\epsilon^{t/2}  +  \alpha_{\ceil{\frac{t}{2}}} \right)\\
    %    &\;\;\; + \frac{2\bar T}{t} \frac{\gamma_{\max}}{\gamma_{\min}} \mathbf{E}[\|\langle \tilde \theta \rangle_{\bar T} -\theta^* \|_2^2 ] 
    %    +  \frac{2 \Psi_2 \alpha_0  C \log^2(\frac{t}{\alpha_0})}{t} \frac{\gamma_{\max}}{\gamma_{\min}}
    %    +  2 \alpha_0 \frac{\gamma_{\max}}{\gamma_{\min}} \frac{\sum_{l = \bar T}^{t} \| \mu_{l} \|_2 }{t}
    %\end{align*}
%    where $\gamma_{\min}$ and $\gamma_{\max}$ are defined in Assumption~\ref{assum:lyapunov}.
%\end{theorem}



 \begin{lemma} \label{lemma:bound_consensus_time-varying_push_SA} 
    Suppose that Assumptions~\ref{assum:A and b} and \ref{assum:step-size} hold and $\{ \bbb{G}_t \}$ is uniformly strongly connected by sub-sequences of length $L$.
    Let $\epsilon_1 = \inf_{t\ge 0}  \min_{i\in\mathcal V} (\hat W_t \cdots \hat W_0 \1_N)^i $. 
    For all $t \ge 0$ and $i \in \mathcal{V}$,
    \begin{align*}
    &\;\;\;\; \| \theta_{t+1}^i - \langle \tilde \theta \rangle_t \|_2 \\
    &\le\frac{8}{\epsilon_1}  \bar\epsilon^t \| \sum_{i=1}^N \tilde \theta_0^i + \alpha_0 A(X_0)\theta_0^i + \alpha_0 b^i(X_0) \|_2+ \alpha_t b_{\max}  \\
    & \;\;\; + \frac{8}{\epsilon_1} \frac{ A_{\max} C_\theta + b_{\max}}{1-\bar\epsilon} \left(  \alpha_0 \bar\epsilon^{t/2}  +  \alpha_{\ceil{\frac{t}{2}}} \right) + \alpha_t  A_{\max} C_\theta ,
\end{align*}
    %\begin{align*}
    %\| \theta_{t+1}^i - \langle \tilde \theta \rangle_t \|_2 
   % &\le\frac{8}{\epsilon_1}  \bar\epsilon^t \| \tilde \Theta_0 \|_1 + \frac{8}{\epsilon_1} \frac{N \sqrt{K} (A_{\max} C_\theta + b_{\max})}{1-\bar\epsilon} \left(  \alpha_0 \bar\epsilon^{t/2}  +  \alpha_{\ceil{\frac{t}{2}}} \right),
%\end{align*}
where $\epsilon_1 > 0$ and $\bar\epsilon \in (0,1)$ satisfy $\epsilon_1 \ge \frac{1}{N^{NL}}$ and $\bar\epsilon \le (1-\frac{1}{N^{NL}})^{1/L}$.
\end{lemma}



\begin{lemma} \label{lemma:eta_limit_Push_SA}
    $\lim_{t \to \infty} \mu_t = \lim_{t \to \infty} \| \rho_t \|_2 =0$ and $\lim_{t \to \infty} \frac{\sum_{k=0}^t \mu_k}{t+1}   = \lim_{t \to \infty} \frac{\sum_{k=0}^t \| \rho_k \|_2}{t+1}  = 0.$
\end{lemma}







\begin{lemma} \label{lemma:bound_average_time-varying_push_SA}
    Suppose that Assumptions~\ref{assum:A and b}--\ref{assum:lyapunov} hold and $\alpha_t = \frac{\alpha_0}{t+1}$. When $ \mu_{t} + \tau(\alpha_t) \alpha_{t-\tau(\alpha_t)} \zeta_8 \le \frac{0.1}{\gamma_{\max}}$ and $\tau(\alpha_t) \alpha_{t-\tau(\alpha_t)} \le \min \{ \frac{ \log2}{A_{\max}},\; \frac{0.1}{\zeta_8 \gamma_{\max}} \}$, we have for $t\ge \bar T$,
%\begin{align*}
%    \mathbf{E}\left[\| \langle \theta \rangle_{t} -\theta^* \|_2^2 \right] 
%    & \le \frac{T_2^*}{t} \frac{\gamma_{\max}}{\gamma_{\min}} \mathbf{E}\left[\|\langle \theta \rangle_{T_2^*} -\theta^* \|_2^2 \right] 
%    +  \frac{\zeta_7 \alpha_0  C \log^2(\frac{t}{\alpha_0})}{t} \frac{\gamma_{\max}}{\gamma_{\min}} +  \alpha_0 \zeta_4 \frac{\gamma_{\max}}{\gamma_{\min}}  \frac{\sum_{l = T_2^*}^{t} \mu_{l}}{t},
%\end{align*}
\begin{align*}
    &\;\;\;\; \mathbf{E}[\|\langle \tilde \theta \rangle_{t+1} -\theta^* \|_2^2 ] \nonumber\\
    & \le \frac{\bar T}{t+1} \frac{\gamma_{\max}}{\gamma_{\min}} \mathbf{E}[\|\langle \tilde \theta \rangle_{\bar T} -\theta^* \|_2^2 ] 
    +  \frac{\zeta_9 \alpha_0  C \log^2(\frac{t+1}{\alpha_0})}{t+1} \frac{\gamma_{\max}}{\gamma_{\min}} \nonumber\\
    &\;\;\; 
     +  \alpha_0 \frac{\gamma_{\max}}{\gamma_{\min}} \frac{\sum_{l = \bar T}^{t+1}  \mu_{l}  }{t+1},
\end{align*}
where $\bar T$ is defined in Appendix~\ref{sec:thmPush_constant}, $\zeta_8$ and $\zeta_9$ are defined in \eqref{eq:definition_Psi12} and \eqref{eq:definition_Psi13}, respectively.
\end{lemma}




We are now in a position to prove Theorem~\ref{thm:bound_time-varying_step_Push_SA}.

\noindent
{\bf Proof of Theorem~\ref{thm:bound_time-varying_step_Push_SA}:}
Note that
    $
        \sum_{i=1}^N \mathbf{E}[\|\theta_{t+1}^i - \theta^*\|_2^2]
         \le 2 \sum_{i=1}^N  \mathbf{E}[\|\theta_{t+1}^i - \langle \tilde \theta \rangle_t \|_2^2 ] + 2 N \mathbf{E} [\| \langle \tilde \theta \rangle_t - \theta^*\|_2^2] .
    $
From Lemmas~\ref{lemma:bound_consensus_time-varying_push_SA} and \ref{lemma:bound_average_time-varying_push_SA}, we have for any $t \ge \bar T$,
\begin{align*}
      &\;\;\;\;\sum_{i=1}^N \mathbf{E}\left[\left\|\theta_{t+1}^i - \theta^*\right\|_2^2\right] \nonumber\\
        & \le \frac{16}{\epsilon_1}  \bar\epsilon^t \mathbf{E}[ \| \sum_{i=1}^N \tilde \theta_0^i + \alpha_0 A(X_0)\theta_0^i + \alpha_0 b^i(X_0) \|_2]  \nonumber\\
    &\;\;\; + 2 \alpha_t  A_{\max} C_\theta + 2 \alpha_t b_{\max} + \frac{2\bar TN}{t} \frac{\gamma_{\max}}{\gamma_{\min}} \mathbf{E}[\|\langle \tilde \theta \rangle_{\bar T} -\theta^* \|_2^2] \\
    & \;\;\; + \frac{16}{\epsilon_1} \frac{ A_{\max} C_\theta + b_{\max}}{1-\bar\epsilon} \left(  \alpha_0 \bar\epsilon^{t/2}  +  \alpha_{\ceil{\frac{t}{2}}} \right) \\
    &\;\;\; +  \frac{2 N \zeta_9 \alpha_0  C \log^2(\frac{t}{\alpha_0})}{t} \frac{\gamma_{\max}}{\gamma_{\min}}
    +  2 \alpha_0 N \frac{\gamma_{\max}}{\gamma_{\min}} \frac{\sum_{l = \bar T}^{t}  \mu_{l}  }{t} \\
    &\le   C_7 \bar\epsilon^t  +  C_8 \left(  \alpha_0 \bar\epsilon^{\frac{t}{2}}  +  \alpha_{\ceil{\frac{t}{2}}} \right)+ C_9 \alpha_t \nonumber\\
    &\;\;\; + \frac{1}{t}\bigg(C_{10} \log^2\Big(\frac{t}{\alpha_0}\Big) + C_{11}\sum_{l = \bar T}^{t}  \mu_{l}  +C_{12}\bigg).
    \end{align*}
This completes the proof.
\hfill $\qed$


%{\color{cyan}Note that, to obtain Theorem~\ref{thm:bound_time-varying_step_Push_SA}, we first needed the properties proposed in Lemma~\ref{lemma:push-sum_pi_intfty} to get the boundedness in Lemma~\ref{lemma:bound_theta}. Then, by using the boundedness, we can obtain the bounds in Lemmas~\ref{lemma:bound_consensus_time-varying_push_SA} and \ref{lemma:bound_average_time-varying_push_SA}, then we can obtain Theorem~\ref{thm:bound_time-varying_step_Push_SA} easily.
%In addition, by using Lemma~\ref{lemma:eta_limit_Push_SA} to Theorem~\ref{thm:bound_time-varying_step_Push_SA}, we can show the convergence of the bound. Besides, Lemma~\ref{lemma:eta_limit_Push_SA} guarantees the convergence of the bounds in Theorem~\ref{thm:bound_time-varying_step_Push_SA}.
%. It is a straightforward step to obtain Theorem~\ref{thm:bound_time-varying_step_Push_SA} from Lemmas~\ref{lemma:bound_consensus_time-varying_push_SA} and \ref{lemma:bound_average_time-varying_push_SA}.}

{\color{black}
We next show the asymptotic performance of \eqref{eq:SA_push-sum}.

%\noindent
{\bf Proof of Theorem~\ref{thm:push_meansq}:}
%{\color{red}Part (1) can be proved by specialization of Theorem~3.1 in \cite{kushner87}.}
From Lemma~\ref{lemma:bound_consensus_time-varying_push_SA}, since $\bar \epsilon \in(0,1)$ and $\alpha_t = \frac{\alpha_0}{t}$, it follows that $\lim_{t\to\infty}\| \theta_{t+1}^i - \langle \tilde \theta \rangle_t \|_2 = 0$, which implies that all $\theta_{t+1}^i$, $i\in \mathcal{V}$, will reach a consensus with $ \langle \tilde \theta \rangle_t $. The update of $ \langle \tilde \theta \rangle_t $ is given in \eqref{eq:update_average_tilde_theta}, which can be treated as a single-agent linear stochastic approximation whose corresponding ODE is \eqref{eq:ode_pushsum}.
In addition, from Theorem~\ref{thm:bound_time-varying_step_Push_SA} and Lemma~\ref{lemma:eta_limit_Push_SA}, 
$\lim_{\rightarrow\infty}\sum_{i=1}^N \mathbf{E}[\|\theta_{t+1}^i - \theta^*\|_2^2]=0$, it follows that $\theta_{t+1}^i$ will converge to $\theta^*$ in mean square for all $i\in\mathcal{V}$.
\hfill $\qed$

\begin{remark}
Finite-time analysis for such a push-based distributed algorithm is challenging. 
Almost all, if not all, the existing push-based distributed optimization works build on the analysis in \cite{nedic}; however, that analysis assumes that a convex combination of the entire history of the states of each agent (and not merely the current state of the agent) is being calculated. This assumption no longer holds in our case.  To obtain a direct finite-time error bound without this assumption, we appeal to a new approach to analyze our push-based SA algorithm by leveraging our consensus-based analyses to establish direct finite-time error bounds for stochastic approximation. 
Specifically, we tailor an absolute probability sequence for the push-based stochastic approximation algorithm and exploit its properties (Lemma~\ref{lemma:push-sum_pi_intfty}). 
\hfill$\Box$
\end{remark}

}

==> simulation.tex <==


\subsection{Simulations} \label{sec:simulation}

%In this section, we numerically validate the finite-time bounds derived in this paper, for both distributed TD($\lambda$) and push-TD($\lambda$), and compare with the existing distributed  TD($\lambda$) results in \cite{doan2019finite}. 
In this section, we numerically validate the finite-time bounds derived in this paper, for both distributed TD($\lambda$) and push-TD($\lambda$), which are the special case of distributed linear stochastic approximation and push-SA, and compare with the existing distributed  TD($\lambda$) results in \cite{doan2019finite}. 
We focus on TD($\lambda$) and TD(0) as the existing distributed TD(0) finite-time analysis in \cite{doan2019convergence} only considers i.i.d. samples.
We focus on TD($\lambda$) and TD(0) as the existing distributed TD(0) finite-time analysis in \cite{doan2019convergence} only considers i.i.d. samples.

The TD setting and multi-agent network are given as follows. Set $\lambda = 0.2 $ and discount factor $\gamma = 0.3$.
Consider an environment with $N=10$ agents and $|\mathcal{S}| = 10$ states. We generated a row stochastic matrix with each entry in $[0, 1]$ and then added a small constant $10^{-5}$ to each element to make sure that the transition matrix satisfies  Assumption~\ref{assum:tranistion}. For each agent $i$ and state pair $(s, s')$, we randomly sampled mean reward $R^i(s,s')$ from $[-3,3]$, and the instantaneous reward $r_t^i$ was randomly sampled from $[R^i(s,a) - 0.5, R^i(s,a) + 0.5]$. 
The dimension of the feature vector $\phi$ was set as $K = 5$. We sampled the entry of $\phi$ from $[0,1]$ while simultaneously guaranteeing that the feature matrix $\Phi$ satisfies Assumption~\ref{assum:feature}.

First, we considered consensus-based algorithm~\eqref{eq:theta update_TD} with time-varying stochastic matrices to show the necessity of  Assumption~\ref{assum:limit_pi}. To this end, we simulated two cases. In this first case, we randomly generated a stochastic matrix at each time step, and thus the corresponding absolute probability sequence  ${\pi_t}$ does not converge. We set the time-varying stepsize as $\alpha_t = 1/t^{0.68}$.
%{\color{red}i don't know why $\alpha_t$ is not $1/t$}
Figure~\ref{fig:Counter}~(\ref{fig:conter_allrowstoc}) shows that in this case the average norm of all agents variables does not converge, implying non-convergence of all agents' states. 
In the second case, we consider a more special case in which the underlying graph changes periodically. In many distributed algorithms like distributed optimization, periodic settings can be regarded as a time-invariant case which thus guarantees convergence. We set the period as 10 and constructed the same set of 10 different stochastic matrices for each period. 
However, Figure \ref{fig:Counter}~(\ref{fig:conter_allrowstoc_period}) shows that even with this periodic setting, the consensus-based algorithm (1) still does not converge, because a periodic sequence of stochastic matrices does not have a convergent absolute probability sequence. 

%\begin{figure}[htbp]
%\centering
%\includegraphics[width=0.5 \linewidth]{Graph/ConterExampleForAllStochasticCase.eps}
%\caption{Necessity of Assumption~\ref{assum:limit_pi}.}
%\label{fig:conter_allrowstoc}
%\end{figure}
%\begin{figure}
%\begin{center}
%\includegraphics[height=4cm]{jcaesar.eps}    % The printed column  
%\caption{Gaius Julius Caesar, 100--44 B.C.}  % width is 8.4 cm.
%\label{fig1}                                 % Size the figures 
%\end{center}                                 % accordingly.
%\end{figure}

%\begin{figure}
%\begin{center}
%\includegraphics[height=4cm]{Graph/ConterExampleForAllStochasticCase.eps}    % The printed column  
%\caption{Random row stochastic matrices}  % width is 8.4 cm.
%\label{fig:conter_allrowstoc}                                 % Size the figures 
%\end{center}                                 % accordingly.
%\end{figure}


\begin{figure}
     \centering
     \begin{subfigure}
         \centering
         \includegraphics[height=4cm]{Graph/ConterExampleForAllStochasticCase.eps}
         \caption{Random row stochastic matrices}
         \label{fig:conter_allrowstoc}
     \end{subfigure}
     \begin{subfigure}
         \centering
         \includegraphics[height=4cm]{Graph/Counter_period.eps}
         \caption{Periodic row stochastic matrices}
         \label{fig:conter_allrowstoc_period}
     \end{subfigure}
        \caption{Non-convergent distributed TD($\lambda$) algorithm (\eqref{eq:theta update_TD}) without Assumption~\ref{assum:limit_pi}.}
        \label{fig:Counter}
\end{figure}


Next, we compared the finite-time bounds derived in this paper with the one in the existing literature \cite{doan2019finite}.
As mentioned earlier, compared with the finite-time analysis of distributed TD($\lambda$) with doubly stochastic matrices in \cite{doan2019finite}, the finite-time analysis in the paper is more general. In the sequel, we will evaluate the theoretical finite-time bounds for both distributed TD($\lambda$) and push-TD($\lambda$).
To illustrate the differences and advantage over \cite{doan2019finite}, for consensus-based distributed TD($\lambda$), we consider the following three settings:
\begin{enumerate}
    \item The first 15 weight matrices are fixed, row stochastic (not doubly stochastic) and the following 85 weight matrices are fixed, doubly stochastic (see Figure~\ref{fig:total} (\ref{fig:M_fixed}) - (\ref{fig:M_time_long})).
    \item All weight matrices are fixed, stochastic matrices, but not doubly stochastic (see Figure~\ref{fig:total} (\ref{fig:D_fixed}), (\ref{fig:D_fixed_long})).
    \item All weight matrices are fixed, doubly stochastic (see Figure~\ref{fig:total} (\ref{fig:ND_fixed}), (\ref{fig:ND_fixed_long})).
\end{enumerate}
In addition, we evaluated the finite-time bound of the push-TD($\lambda$) algorithm with a fixed, column stochastic weight matrix (see Figure~\ref{fig:P_time_total}).

Figure~\ref{fig:total} (\ref{fig:M_fixed}), \ref{fig:total} (\ref{fig:M_time}) and \ref{fig:total} (\ref{fig:D_fixed}) show that the bounds proposed in this paper 
%\eqref{eq:finite-time bound_TD_fixed}, \eqref{eq:finite-time bound_TD_timevarying} 
and \cite{doan2019finite} can be used to bound the actual error. However, the stating time for the bounds proposed in this paper 
%in \eqref{eq:finite-time bound_TD_fixed} and \eqref{eq:finite-time bound_TD_timevarying} 
are earlier than those in \cite{doan2019finite}. 

Figure~\ref{fig:total} (\ref{fig:M_fixed_long}) and \ref{fig:total} (\ref{fig:D_fixed_long}) show both bounds in this paper %\eqref{eq:finite-time bound_TD_fixed} 
and \cite{doan2019finite} will converge to some fixed values when the stepsize is fixed. These values are listed and compared in  Table~\ref{table:converge value}. Figure~\ref{fig:total}(\ref{fig:M_time_long}) shows that both the bounds in this paper %\eqref{eq:finite-time bound_TD_timevarying} 
and \cite{doan2019finite} will converge to zero for the time-varying stepsize.

\begin{table}[t]
\centering
\caption{Comparison of the asymptotic bounds}
\begin{tabular}{ |p{3cm}|p{2cm}|p{2cm}|  } 
 %\hline
 %\multicolumn{3}{|c|}{Bound at Time$=\infty$ } \\
 \hline
  & Bound in this paper & Bound in \cite{doan2019finite}\\
 \hline
 Mixed stochastic matrices$^*$ $+$ fixed stepsize   & 88.1653    & 114.1386\\
 \hline 
 Mixed stochastic matrices $+$ time-varying stepsize &   0  & 0\\
 \hline 
 All doubly stochastic matrices $+$ fixed stepsize & 881.5952 & 1141.4\\
 \hline 
 All non-doubly, stochastic matrices $+$ fixed stepsize    & 241.6035 & NA \\
 \hline 
 All column stochastic matrices (push-TD) $+$ time-varying stepsize &   0  & NA \\
 \hline 
\end{tabular}
\label{table:converge value}
\footnotesize{$^*$A set of mixed stochastic matrices contains both doubly and non-doubly ones}
\end{table}

Figure~\ref{fig:total} (\ref{fig:ND_fixed}) and \ref{fig:total} (\ref{fig:ND_fixed_long}) show that the bound in \cite{doan2019finite} can not be (directly) applied to the stochastic (not doubly stochastic) weight matrix case. In addition, Figure \ref{fig:total} (\ref{fig:ND_fixed_long}) shows that the bound in \eqref{eq:finite-time bound_TD_fixed} will converge to some fixed value when the stepsize is fixed, which is given in Table~\ref{table:converge value}. 

Figure~\ref{fig:P_time_total} shows that the push-TD($\lambda$) algorithm will converge to the optimal point in the long run, and the bound in \eqref{eq:finite-time bound_PushTD} can be used to bound the actual error. It is worth emphasizing that the bound in \cite{doan2019finite} cannot be applied for this case.






%{\color{red}make sure the figures are easy to read}





\begin{figure}
     \centering
     \begin{subfigure}
         \centering
         \includegraphics[height=4cm]{Graph/Mixing Graph_fixed stepsize.eps}
         \caption{Mixed   stochastic  matrices (fixed stepsize)}
         \label{fig:M_fixed}
     \end{subfigure}
     \begin{subfigure}
         \centering
         \includegraphics[height=4cm]{Graph/Mixing Graph_fixed stepsize_long time.eps}
         \caption{Mixed   stochastic  matrices (fixed stepsize)}
         \label{fig:M_fixed_long}
     \end{subfigure}
        %\caption{Finite-time Bound for Mixing Graph (Fixed Stepsize).}
        %\label{fig:M_fixed_total}
     \centering
     \begin{subfigure}
         \centering
         \includegraphics[height=4cm]{Graph/Mixing Graph_timevarying stepsize.eps}
         \caption{Mixed   stochastic  matrices (time-varying stepsize)}
         \label{fig:M_time}
     \end{subfigure}
     \begin{subfigure}
         \centering
         \includegraphics[height=4cm]{Graph/Mixing Graph_timevarying stepsize_long time.eps}
         \caption{Mixed   stochastic  matrices (time-varying stepsize)}
         \label{fig:M_time_long}
     \end{subfigure}
        %\caption{Finite-time Bound for Mixing Graph (Time-varying Stepsize).}
        %\label{fig:M_time_total}
     \centering
     \begin{subfigure}
         \centering
         \includegraphics[height=4cm]{Graph/Doubly Graph_fixed stepsize.eps}
         \caption{All doubly stochastic matrices (fixed stepsize)}
         \label{fig:D_fixed}
     \end{subfigure}
     \begin{subfigure}
         \centering
         \includegraphics[height=4cm]{Graph/Doubly Graph_fixed stepsize_long time.eps}
         \caption{All doubly stochastic matrices (fixed stepsize)}
         \label{fig:D_fixed_long}
     \end{subfigure}
        %\caption{Finite-time Bound for Doubly Graph (Fixed Stepsize).}
        %\label{fig:D_fixed_total}
     \centering
     \begin{subfigure}
         \centering
         \includegraphics[height=4cm]{Graph/Non-Doubly Graph_fixed-stepsize.eps}
         \caption{All non-doubly, stochastic matrices (fixed stepsize)}
         \label{fig:ND_fixed}
     \end{subfigure}
     \begin{subfigure}
         \centering
         \includegraphics[height=4cm]{Graph/Non-Doubly Graph_fixed stepsize_long time.eps}
         \caption{All non-doubly, stochastic matrices (fixed stepsize)}
         \label{fig:ND_fixed_long}
     \end{subfigure}
        \caption{Finite-time bounds for consensus-based TD($\lambda$) (\eqref{eq:theta update_TD}).}
        \label{fig:total}
\end{figure}
%\subsection{Push-sum}
\begin{figure}
     \centering
     \begin{subfigure}
         \centering
         \includegraphics[height=4cm]{Graph/PushSum_timevarying stepsize.eps}
         \label{fig:P_time}
     \end{subfigure}
     \begin{subfigure}
         \centering
         \includegraphics[height=4cm]{Graph/PushSum_timevarying stepsize_long time.eps}
         \label{fig:P_time_long}
     \end{subfigure}
        \caption{Finite-time bounds for push-TD($\lambda$) (\eqref{eq:td_push-sum}) with time-varying stepsizes.}
        \label{fig:P_time_total}
\end{figure}
%\subsection{Mixing Graph}

%\begin{figure}[htbp]
%     \centering
%     \begin{subfigure}[htbp]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Graph/Mixing Graph_fixed stepsize.eps}
%         \label{fig:M_fixed}
%         \caption{Mixing Graph(Fixed Stepsize)}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[htbp]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Graph/Mixing Graph_fixed stepsize_long time.eps}
%         \label{fig:M_fixed_long}
%         \caption{Mixing Graph(Fixed Stepsize)}
%     \end{subfigure}
%        \caption{Finite-time Bound for Mixing Graph (Fixed Stepsize).}
%        \label{fig:M_fixed_total}
%\end{figure}

%\begin{figure}[htbp]
%     \centering
%     \begin{subfigure}[htbp]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Graph/Mixing Graph_timevarying stepsize.eps}
%         \label{fig:M_time}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[htbp]{0.45\textwidth}
%         \centering
 %        \includegraphics[width=\textwidth]{Graph/Mixing Graph_timevarying stepsize_long time.eps}
%         \label{fig:M_time_long}
%     \end{subfigure}
%        \caption{Finite-time Bound for Mixing Graph (Time-varying Stepsize).}
%        \label{fig:M_time_total}
%\end{figure}

%\subsection{Doubly Graph}

%\begin{figure}[htbp]
%     \centering
%     \begin{subfigure}[htbp]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Graph/Doubly Graph_fixed stepsize.eps}
%         \label{fig:D_fixed}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[htbp]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Graph/Doubly Graph_fixed stepsize_long time.eps}
%         \label{fig:D_fixed_long}
%     \end{subfigure}
%        \caption{Finite-time Bound for Doubly Graph (Fixed Stepsize).}
%        \label{fig:D_fixed_total}
%\end{figure}

%\subsection{Non-Doubly Graph}

%\begin{figure}[htbp]
%     \centering
%     \begin{subfigure}[htbp]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Graph/Non-Doubly Graph_fixed stepsize.eps}
%         \label{fig:ND_fixed}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[htbp]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Graph/Non-Doubly Graph_fixed stepsize_long time.eps}
%         \label{fig:ND_fixed_long}
%     \end{subfigure}
%        \caption{Finite-time Bound for Non-Doubly Graph (Fixed Stepsize).}
%        \label{fig:ND_fixed_total}
%\end{figure}
%\subsection{Push-sum}
%\begin{figure}[htbp]
%     \centering
%     \begin{subfigure}[htbp]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Graph/PushSum_timevarying stepsize.eps}
%         \label{fig:P_time}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[htbp]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Graph/PushSum_timevarying stepsize_long time.eps}
%         \label{fig:P_time_long}
%     \end{subfigure}
%        \caption{Finite-time Bound for Push-sum Algorithm (Time-varying Stepsize).}
%        \label{fig:P_time_total}
%\end{figure}

In summary, from the figures and Table~\ref{table:converge value}, we can see that (1) our consensus-based TD($\lambda$) can be applied to more general time-varying row stochastic matrices cases; though our finite-time bound is looser at the beginning period, it can be applied at an earlier time instant and has a tighter limiting bound, compared with \cite{doan2019finite}; and (2) our push-based TD($\lambda$) expands the applicability of the existing distributed TD learning, as it can work for any time-varying directed graphs as long as they are uniformly strongly connected, without any restrictive assumptions such as Assumption~6 in our consensus-based one and the doubly stochasticity assumption in \cite{doan2019finite}.
